AnalogNets: ML-HW Co-Design of Noise-robust TinyML Models and Always-On Analog Compute-in-Memory Accelerator

Always-on TinyML perception tasks in IoT applications require very high energy efficiency. Analog compute-in-memory (CiM) using non-volatile memory (NVM) promises high efficiency and also provides self-contained on-chip model storage. However, analog CiM introduces new practical considerations, including conductance drift, read/write noise, fixed analog-to-digital (ADC) converter gain, etc. These additional constraints must be addressed to achieve models that can be deployed on analog CiM with acceptable accuracy loss. This work describes $\textit{AnalogNets}$: TinyML models for the popular always-on applications of keyword spotting (KWS) and visual wake words (VWW). The model architectures are specifically designed for analog CiM, and we detail a comprehensive training methodology, to retain accuracy in the face of analog non-idealities, and low-precision data converters at inference time. We also describe AON-CiM, a programmable, minimal-area phase-change memory (PCM) analog CiM accelerator, with a novel layer-serial approach to remove the cost of complex interconnects associated with a fully-pipelined design. We evaluate the AnalogNets on a calibrated simulator, as well as real hardware, and find that accuracy degradation is limited to 0.8$\%$/1.2$\%$ after 24 hours of PCM drift (8-bit) for KWS/VWW. AnalogNets running on the 14nm AON-CiM accelerator demonstrate 8.58/4.37 TOPS/W for KWS/VWW workloads using 8-bit activations, respectively, and increasing to 57.39/25.69 TOPS/W with $4$-bit activations.

==> sections/hw_design_exploration.tex <==
% \section{Depthwise Convolutional Layers: Deployment of MicroNet-KWS-S on a $1024 \times 512$ differential crossbar array}
% \label{sec:dwcl_deployment}
% \begin{figure*}[bp!]
%     \centering
%     \begin{minipage}{0.8\columnwidth}
%     \centering
%     \subfloat[MicroNet-KWS-S deployment on a $1024 \times 512$ NVM crossbar tile.]{\label{fig:depth_wise_kws:a}\includegraphics[width=0.98\columnwidth]{figs/dwsc_layers/mapping_m_0_r_1024_c_512.pdf}}
%     \end{minipage}%
%     \begin{minipage}{1.2\columnwidth}
%     \centering
%     \subfloat[MicroNet-KWS-S deployment on multiple $128 \times 128$ NVM crossbar  tiles.]{\label{fig:depth_wise_kws:b}\includegraphics[width=0.98\columnwidth]{figs/dwsc_layers/mapping_m_0_r_128_c_128.pdf}}
%     \qquad
%     \centering
%     \subfloat[MicroNet-KWS-S deployment on multiple $64 \times 64$ NVM crossbar  tiles.]{\label{fig:depth_wise_kws:c}\includegraphics[width=0.98\columnwidth]{figs/dwsc_layers/mapping_m_0_r_64_c_64.pdf}}
%     \end{minipage}\par\medskip
	
%     \caption{MicroNet-KWS-S deployment on a $1024 \times 512$ differential crossbar array. Depthwise convolutional layers are represented using semi-transparent colors, while their effective weights --non-zero weights contributing to the layer computation-- are depicted as solid diagonal areas. Layers represented with solid colors correspond to regular 2-dimensional layers. }
%     \label{fig:depth_wise_kws}
% \end{figure*}

% As described in Section~\ref{sec:models}, depthwise  convolutional layers (DWCL)  are  not  suitable  for  CiM analog architectures, attending both at effective utilization and SNR contributions. 
% This effect is clearly visible in Figure~\ref{fig:depth_wise_kws:a}, which magnifies how DWCLs are inefficient compared against normal convolutional layers. The weights deployment map describes how \emph{MicroNet-KWS-S} NN reaches an effective utilization for MicroNet-KWS-S as low as $~9\%$.
% A possible solution to better use the NVM crossbar area resources require splitting the large DWCL GEMM operations into smaller ones operating in a sequential way. Figures~\ref{fig:depth_wise_kws:b} and ~\ref{fig:depth_wise_kws:c} manifest how the crossbar area utilization improves inversely to the maximum size of the split GEMM operation. The main drawback associated with this technique is the layer latency, which due to the sequential operation scheme gets magnified.
% Table \ref{table:dwcl} summarizes the utilization/latency increment trade-off.
% \begin{table}[ht]
% \caption{Resource vs latency comparison for the deployment of MicroNet-KWS-S as an example of NN heavily relying on Depthwise convolutional layers.}
% \centering
% \begin{tabular}{|c|c|c|c|}
% \hline
% \textbf{Crossbar}               & \textbf{$1024 \times 512$} & $128 \times 128$ & $64 \times 64$ \\
% \hline
% \textbf{Eff. Utilization}    & $9\%$            & $40\%$          & $66 \%$ \\
% \hline
% \textbf{Inference/s}    & $4122$            & $1467$          & $642$ \\
% \hline
% \end{tabular}
% \label{table:dwcl}
% \end{table}

\section{Hardware Design Space Exploration}
\label{sec:appendix_hw}
Section~\ref{sec:hw_arch} described the proposed accelerator architecture, composed of \emph{a)} a $1024 \times 512$ differential crossbar array assisted by DAC/ADC periphery, and \emph{b)} the activation processing and storage pipeline.
The PCM crossbar dimensions were specified to support the deployment of either of AnalogNet-KWS or Analog-VWW.
However, the sizing of the periphery supporting the main crossbar will influence the PPA characteristics of the accelerator.
On the one hand, a larger number of DACs/ADCs deployed in parallel would potentially maximize the crossbar utilization leading to \emph{a)} shorter latency and increased throughput, \emph{b)} improved efficiency. On the other hand, deploying more converters would lead to a significant increment in the accelerator area.
Being area a critical constraint in IoT systems, in the present section we summarize the analysis after performing the design space exploration that lead to the final accelerator design involving $1024$ DACs, $128$ ADCs and $32$ FP units assisting the main crossbar. Therefore the AON-CiM accelerator follows a multiplexing scheme M$1$-M$4$-M$4$ --one DAC supporting each crossbar row, one ADC multiplexed every four crossbar columns, and 1 FP unit multiplexed each four ADCs.
First, the computation of a single layer can be decomposed into multiple sub-stages is discussed. Second the multiplexing of data converter periphery and activations processing circuitry is analyzed.
Finally, the PPA characteristics after the deployment of the same AnalogNets workloads on different crossbar configurations --bigger versus smaller sub-arrays-- are presented.

\subsection{Deployment of a Larger Layer into Smaller Crossbar Arrays or Smaller Crossbar Subsections}

\todo{Didn't entirely follow this paragraph - let's discuss?}

A large GEMM operation may not fit into a single crossbar array requiring to be split and deployed into many crossbars, combining the MAC operation outputs of each of the crossbars involved that hold the partial computations.
This operation can be accomplished sequentially (one partial computation at a time) or in parallel.
But similarly, and as presented in Section~\ref{sec:dwcl_deployment}, we may split a large GEMM matrix into smaller sub-matrices that could be deployed in a single crossbar and computed in a sequential manner.
The exercise of split-mapping the NN to smaller crossbar arrays is equivalent to selectively activating different sub-regions on a larger array and using less periphery resources.

The scheme in which the computation of a single vector-matrix multiplication involving $M \times N$ weights can be serialized in multiple operations using $M'\times N'$ weights, $M'<M, N'<N$ has different direct applications.
The first one has already be discussed: the more efficient the deployment of depthwise convolutional layers.
The second one refers to systems limited by the accelerator area. 
IoT systems may require reducing the accelerator silicon by reducing the number of DACs or ADCs.
The data-conversion periphery can be multiplexed, and therefore the computation of larger layers is still feasible at the expense of \emph{a)} latency increase and \emph{b)}throughput reduction.
The third application regards the deployment of DNN composed of layers with very different geometry after the GEMM unrolling.
As described in Sections~\ref{sec:analog:adc_gain} and~\ref{sec:models:adc_gain} --the ADC physical and modeling implementation respectively, the dynamic range of the signals flowing through the system and the constraints of the scaling operations between filters and layers can potentially compromise the system accuracy. This challenge is even more dramatic as the conductance drift compensation modules in charge of limiting the accuracy degradation through time are quite sensitive to these scaling factors \cite{Joshi2020, aljameh-hermes-vlsi2021}.
A potential solution for DNN whose accuracy is highly impacted by this issue comes from the splitting of the taller GEMM layers into sub-regions, inducing a better control on the signals dynamic range and overcoming the challenge at the expense of an increased computation latency. 

\subsection{Periphery Circuitry Multiplexing}

As described in Section~\ref{sec:models}, the deployment of AnalogNet-KWS requires the use of tall layers that almost require the entire crossbar area (and DAC associated resources) for the activated columns. Therefore we decided to fully support the PCM crossbar with DACs interfaces, meaning that by deploying $1024$ DACs no DAC requires to be multiplexed --scheme M$1$.

On the contrary, and by an inspection of the deployment maps presented in Figure~\ref{fig:mapping}, the number of ADCs required by each layer is far from the $512$ columns present in the crossbar.
Therefore, the impact on the area, throughput, energy and efficiency of the different ADCs multiplexing schemes for the peak --$100\%$ crossbar utilization-- and the proposed workloads has been analyzed.
We consider then a  M$1$-M$X$-M$1$ periphery/activations circuitry multiplexing scheme, where the same number of FP units for activations/scaling operations as ADCs are present.
Table \ref{table:hw_periphery_mux} summarizes the findings.
First, we can see how the peak throughput and peak efficiency is directly proportional to the number of ADCs working in parallel.
However, it can also be noted how the deployment of this extra periphery has a considerable impact on the accelerator area.

An important finding is that the mean throughput and efficiency is workload related, meaning that depending on the workloads we target our accelerator to run, we can optimize the area required with almost no loss in throughput or energy efficiency.
The results highlight how for the proposed workloads we are able to maintain both throughput and energy efficiency while considerably reducing the accelerator area.
The deployment of M$1$-M$4$-M$1$ multiplexing scheme requires $20\%$ less area than M$1$-M$1$-M$1$.
\begin{table*}[t]
\caption{
PPA characteristics for different AON Accelerators varying the periphery supporting the $1024 \times 512$ differential crossbar.
The different ADC multiplexing modes correspond to M$1$-512 ADCs, M$2$-256 ADCs, M$4$-128 ADCs. Each of the ADC multiplexing modes contains the same number of FP units for activations/scaling operations as ADCs are present. Therefore the total multiplexing mode is M$1$-M$X$-M$1$.
}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}

\hline
\multicolumn{2}{|c|}{\textbf{ADC MUX}} &\multicolumn{3}{|c|}{\textbf{M1}} & \multicolumn{3}{|c|}{\textbf{M2}}& \multicolumn{3}{|c|}{\textbf{M4}} \\
\hline
\multicolumn{2}{|c|}{\textbf{Total Area [mm$^2$]}} &\multicolumn{3}{|c|}{4.11} & \multicolumn{3}{|c|}{3.60}& \multicolumn{3}{|c|}{3.34} \\
\hline
\multicolumn{2}{|c|}{\textbf{Full Utilization}} & \textbf{4b Act.} & \textbf{6b Act.} & \textbf{8b Act.} & \textbf{4b Act.} & \textbf{6b Act.} & \textbf{8b Act.}& \textbf{4b Act.} & \textbf{6b Act.} & \textbf{8b Act.} \\
\hline
\multicolumn{2}{|c|}{MAX TOPS} & $104.85$    & $30.84$  & $8.06$    & $52.43$ & $15.42$ & $4.03$   & $26.21$ & $7.71$ & $2.02$\\ 
\hline
\multicolumn{2}{|c|}{MAX TOPS/W} & $176.34$ & $91.12$ & $31.37$     & $148.26$ & $68.37$ & $21.81$ & $112.44$ & $45.55$ & $13.55$ \\ 
\hline
\hline
\hline
\multicolumn{2}{|c|}{\textbf{ADC MUX}} &\multicolumn{3}{|c|}{\textbf{M1}} & \multicolumn{3}{|c|}{\textbf{M2}}& \multicolumn{3}{|c|}{\textbf{M4}} \\
\hline
\multicolumn{2}{|c|}{\textbf{Workload}} & \textbf{4b Act.} & \textbf{6b Act.} & \textbf{8b Act.} & \textbf{4b Act.} & \textbf{6b Act.} & \textbf{8b Act.}& \textbf{4b Act.} & \textbf{6b Act.} & \textbf{8b Act.} \\
\hline
\multirow{2}{*}{Mean TOPS} 
    & KWS & $7.8$  & $2.296$  & $0.6$  &  $7.8$ & $2.29$ & $0.6$ &  $7.8$ & $2.29$ & $0.6$ \\
    & VWW & $1.04$ & $0.30$   & $0.08$ &  $1.04$ & $0.3$ & $0.08$&  $0.98$ & $0.29$ & $0.075$ \\ 
\hline
\multirow{2}{*}{Mean TOPS/W} 
    & KWS & $78.50$  & $30.60$  & $8.94$ & $78.50$ & $30.60$ & $8.94$ & $60.54$ & $27.43$ & $8.65$ \\
    & VWW & $34.68$  & $15.05$  & $4.73$ & $31.627$ & $14.44$ & $4.66$& $28.97$ & $13.58$ & $4.45$ \\ 
\hline
\multirow{2}{*}{Inf./Sec} 
    & KWS & $100908$ & $29678$ & $7762$ & $100908$ & $29678$ & $7762$  & $100908$ & $29678$ & $7762$  \\
    & VWW & $14609$  & $4296$  & $1123$ & $14609$  & $4296$  & $1123$ & $13827$ & $4066$ & $1063$\\ 
\hline
\multirow{2}{*}{Energy/Inf.} 
    & KWS & $1.22\mu$J & $2.63\mu$J & $8.22\mu$J  & $1.22\mu$J & $2.63\mu$J & $8.22\mu$J  &$1.22\mu$J & $2.63\mu$J & $8.22\mu$J \\
    & VWW & $2.69\mu$J & $5.07\mu$J & $14.20\mu$J & $2.69\mu$J & $5.07\mu$J & $14.20\mu$J & $2.79\mu$J & $5.43\mu$J & $15.6\mu$J \\ 
\hline
\end{tabular}
%}
\label{table:hw_periphery_mux}
\end{table*}

\subsection{Activation Circuitry Multiplexing}
\begin{figure*}[bp!]
    \centering
	\subfloat[Activation/Scaling FP operations during inference process, for adjusted, over-adjusted, and sub-adjusted pipelines]{\centering
	\includegraphics[width=\textwidth]{figs/operation_new.pdf}
	\label{fig:operation_new}}
    \qquad	
    \centering
	\subfloat[AnalogNets-KWS efficiency, throughput, area and latency]{\centering
	\includegraphics[width=0.98\columnwidth]{figs/kws_fp_exploration.pdf}}
    \qquad	
	\subfloat[AnalogNets-VWW efficiency, throughput, area and latency]{\centering
	\includegraphics[width=0.98\columnwidth]{figs/vww_fp_exploration.pdf}}
    \caption{
    Inference pipeline detaining the SRAM, PCM crossbar and activation/scaling FP operation stages.
    Design space exploration for different activation precision and analyzing the area, throughput and efficiency implications of varying the number of parallel FP multipliers.
    }
    \label{fig:ppa_fp_exploration}
\end{figure*}

As described in the previous section, the floating point (FP) units involved in the computation of the activation and scaling stages --Figure \ref{fig:accelerator}-- can be multiplexed in order to minimize its impact on the accelerator area while keeping constant the throughput and energy efficiency for the required workloads.
The diagram on Figure~\ref{fig:operation_new} describes the inference pipeline focusing on the different modules involved. We catalogue a pipeline as adjusted if the periphery/crossbar latency matches the latency of the the activation/scaling FP operations and SRAM writes. Under those conditions the latency of the pipeline is minimized and the resources use is maximized in the most efficient way.
However, if the periphery/crossbar latency is much shorter than the FP operations latency, we would impose \emph{IDLE} states on the pipeline as described in the figure.
Taking into account that the periphery/crossbar latency is a function of the precision of the DACs/ADCs, it is important to explore the minimum number of FP units is able to provide the required throughput.

As described before, the maximum throughput achievable is a function of the workload being accelerated.
For such purpose the design space exploration of the FP units multiplexing schemes and its effects on the accelerator PPA was carried out.
The number of FP units was varied, therefore studying the characteristics of M$1$-M$4$-M$X$ systems.
Figure~\ref{fig:ppa_fp_exploration} summarizes the system PPA characteristics when operating at different activations precision.
The results showed that $32$ FP units running in parallel are the optimum number for maximizing the accelerator performance for both KWS and VWW applications while keeping the area reduced.

Finally, to illustrate the effects that an unbalanced pipeline has on the overall throughput/efficiency of the system, Figure\ref{fig:pareto_exploration} analyzes the characteristics for each layer geometry under different FP multiplexing scheme, highlighting the importance of a tuned design over a naive one.

\begin{figure*}[bp!]
    \centering
	\subfloat[M$1$-M$4$-M$32$ multiplexing scheme.]{\centering
	\includegraphics[width=0.31\textwidth]{figs/FP_4.pdf}
	\label{fig:operation_new}}
    \centering
	\subfloat[M$1$-M$4$-M$8$ multiplexing scheme.]{\centering
	\includegraphics[width=0.31\textwidth]{figs/FP_16.pdf}}
	\subfloat[M$1$-M$4$-M$4$ multiplexing scheme.]{\centering
	\includegraphics[width=0.31\textwidth]{figs/FP_32.pdf}}
    \caption{
    Design space exploration of different layer geometries for M$1$-M$4$-M$32$, M$1$-M$4$-M$8$ and M$1$-M$4$-M$4$ multiplexing schemes, providing the throughput/efficiency pareto for the deployed layers.
    }
    \label{fig:pareto_exploration}
\end{figure*}

\subsection{Layer by Layer PPA Analyses for  M$1$-M$4$-M$4$ AON Accelerator}

In this section we analyze the throughput and efficiency achieved after the deployment of the proposed AnalogNet workloads on the M$1$-M$4$-M$4$ AON Accelerator, whose main PPA characteristics were described in Section~\ref{sec:results}.
\begin{figure*}[h]
    \centering
	\subfloat[AnalogNets-KWS efficiency vs throughput]{\centering
	\includegraphics[width=0.98\columnwidth]{figs/baseline/analognet-kws_big/l_eff_TOPS_l_eff_mean_TOPS_W.pdf}}
    \qquad	
    \subfloat[AnalogNets-VWW efficiency vs throughput]{\centering
    \includegraphics[width=0.98\columnwidth]{figs/baseline/analognet-vww_big/l_eff_TOPS_l_eff_mean_TOPS_W.pdf}}
%     \caption{
%     Layer-wise efficiency and throughput decomposition for both analyzed workloads after its deployment on a single $1024 \times 512$ differential crossbar assisted by $1024$ DACs, $256$ ADCs and $32$ FP units.
%     }
%     \label{fig:ppa_1024_0}
% \end{figure*}

% \begin{figure*}[h]
%     \centering
    % \qquad	
	\subfloat[AnalogNets-VWW efficiency vs area]{\centering
	\includegraphics[width=0.98\columnwidth]{figs/baseline/analognet-kws_big/l_area_l_eff_mean_TOPS_W.pdf}}
    \qquad	
    \subfloat[AnalogNets-KWS efficiency vs area]{\centering
    \includegraphics[width=0.98\columnwidth]{figs/baseline/analognet-vww_big/l_area_l_eff_mean_TOPS_W.pdf}}
    \caption{
    Layer-wise throughput, efficiency and area decomposition for both analyzed workloads after its deployment on a single $1024 \times 512$ differential crossbar assisted by $1024$ DACs, $256$ ADCs and $32$ FP units.
    }
    \label{fig:ppa_1024_1}
\end{figure*}
Figure \ref{fig:ppa_1024_1} extends the results initially presented in Figure~\ref{fig:tops-topsw-for-layers} describing the different layers efficiency as a function of its throughput and area for the three considered activations precision.
In the diagrams, the size of the marker relates to the number of weights present in the layer.
This study reveals the direct relation between the size of the layer, the number of performed operations, and the layer performance.
Similarly, the throughput and power implications of higher precision periphery is established, and compared against the maximum achievable efficiencies for each mode --dotted lines-- on this M$1$-M$4$-M$4$ AON Accelerator.

\subsection{Deployment on Smaller Arrays}

\begin{figure}[tp!]
    \centering
  \begin{subfigure}[b]{\columnwidth}
    \includegraphics[width=\linewidth]{figs/deployment_256_256/analognet-kws_small/mapping_m_0_r_256_c_256.pdf}
    \caption{AnalogEdge-KWS mapping requiring $6$ $256 \times 256$ differential crossbars.}
    \label{fig:mapping_kws_256}
  \end{subfigure}
  \hfill %%
  \begin{subfigure}[b]{\columnwidth}
    \includegraphics[width=\linewidth]{figs/deployment_256_256/analognet-vww_small/mapping_m_0_r_256_c_256.pdf}
    \caption{AnalogEdge-VWW mapping requiring $6$ $256 \times 256$ differential crossbars.}
    \label{fig:mapping_vww_256}
  \end{subfigure}
    \caption{
    \emph{AnalogEdge-KWS} and \emph{AnalogEdge-VWW} mapping to multiple $256 \times 256$ crossbar with differential columns, achieving $76.5\%$ and $77.2\%$ utilization, respectively.
    }
    \label{fig:mapping-small-array}
\end{figure}

A final study is presented in which the trade-off between area and throughput is explored by reducing the size of the active layers by splitting them in sub-matrices requiring less periphery.
This exercise compares the single $1024 \times 512$ M$1$-M$4$-M$4$ differential crossbar accelerator  --up to $1024$ DACs, $128$ ADCs and $32$ FP units-- against one composed of multiple  $256 \times 256$ working in a M$1$-M$2$-M$4$ multiplexing scheme --up to $256$ DACs, $128$ ADCs and $32$ FP units.
Figure \ref{fig:mapping-small-array} describes the layer mapping on the multiple $256 \times 256$ crossbars, noticeably altering the initial maps seen in Figure \ref{fig:mapping}.
The reduction in the number of DACs had a limited impact on the accelerator area --$4\%$ area decrease.
On the carried out design exploration experiments the periphery multiplexing reported the most impact on the accelerator area, followed by the number of FP units present in the design.


\begin{table*}[bp!]
\caption{
PPA characteristics of the proposed accelerator, and comparison against an alternative multi-tile implementation. The table describes \emph{a)} the maximum efficiency and throughput numbers correspond to a single layer utilizing $100\%$ of the resources; and \emph{b)}, the throughput and efficiency for the studied workloads. A clear trend between the number of parallel \emph{ops} (defined as either a multiplication or an accumulation) and the crossbar size is established. In both larger/smaller tiling approaches, a maximum of $128$ ADCs are deployed, imposing M$4$ and M$2$ muxing respectively.
}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|}

\hline
\multicolumn{2}{|c|}{\textbf{Crossbar Size (Differential columns)}} & \multicolumn{3}{|c|}{\textbf{Single $1024 \times 512$}} & \multicolumn{3}{|c|}{\textbf{Multiple $256 \times 256$}} \\
\multicolumn{2}{|c|}{\textbf{DAC-ADC-FPu Multiplexing Scheme}} &\multicolumn{3}{|c|}{\textbf{M$1$-M$4$-M$4$}} & \multicolumn{3}{|c|}{\textbf{ M$1$-M$2$-M$4$}} \\\hline
\multicolumn{2}{|c|}{\textbf{Periphery Area [mm$^2$]}} & \multicolumn{3}{|c|}{0.25} & \multicolumn{3}{|c|}{0.11}  \\
\hline
\multicolumn{2}{|c|}{\textbf{At Full Utilization}} & \textbf{4b Act.} & \textbf{6b Act.} & \textbf{8b Act.} & \textbf{4b Act.} & \textbf{6b Act.} & \textbf{8b Act.} \\
\hline
\multicolumn{2}{|c|}{MAX TOPS} & $26.21$    & $7.71$  & $2.02$    & $6.55$ & $1.93$ & $0.50$\\ 
\hline
\multicolumn{2}{|c|}{MAX TOPS/W} & $112.44$ & $45.55$ & $13.55$ & $45.98$ & $24.50$ & $8.66$\\ 
\hline
\hline
\hline
\multicolumn{2}{|c|}{\textbf{Crossbar Size (Differential columns)}} &\multicolumn{3}{|c|}{\textbf{Single $1024 \times 512$}} & \multicolumn{3}{|c|}{\textbf{Multiple $256 \times 256$}} \\
\multicolumn{2}{|c|}{\textbf{DAC-ADC-FPu Multiplexing Scheme}} &\multicolumn{3}{|c|}{\textbf{M$1$-M$4$-M$4$}} & \multicolumn{3}{|c|}{\textbf{ M$1$-M$2$-M$4$}} \\
\hline
\multicolumn{2}{|c|}{\textbf{Workload}} & \textbf{4b Act.} & \textbf{6b Act.} & \textbf{8b Act.} & \textbf{4b Act.} & \textbf{6b Act.} & \textbf{8b Act.} \\
\hline
NVM Crossbar & KWS & $57.3\%$ & $57.3\%$ & $57.3\%$ & $76.5\%$ & $76.5\%$ & $76.5\%$ \\
Utilization  & VWW & $57.3\%$ & $67.5\%$ & $67.5\%$ & $77.2\%$ & $77.2\%$ & $77.2\%$ \\ 
\hline
\multirow{2}{*}{Mean TOPS} 
    & KWS & $7.8$  & $2.296$  & $0.6$  &  $3.65$ & $1.07$ & $0.28$ \\
    & VWW & $0.98$ & $0.29$ & $0.075$ & $0.98$ & $0.29$ & $0.07$ \\ 
\hline
\multirow{2}{*}{Mean TOPS/W} 
    & KWS & $57.39$  & $26.76$  & $8.58$ & $35.43$ & $20.30$ & $7.57$ \\
    & VWW & $25.69$  & $12.82$  & $4.37$ & $25.53$ & $12.74$ & $4.34$ \\ 
\hline
\multirow{2}{*}{Inf./Sec} 
    & KWS & $100908$ & $29678$ & $7762$ & $47258$ & $13899$ & $3635$ \\
    & VWW & $13827$  & $4066$  & $1063$ & $13734$ & $4039$  & $1056$ \\ 
\hline
\multirow{2}{*}{Energy/Inf.} 
    & KWS & $1.22\mu$J & $2.63\mu$J & $8.22\mu$J  & $2.02\mu$J & $3.70\mu$J  & $10.4\mu$J \\
    & VWW & $2.79\mu$J & $5.42\mu$J & $15.60\mu$J & $2.82\mu$J & $5.47\mu$J & $15.7\mu$J \\ 
\hline
\end{tabular}
%}
\label{table:hw_big_vs_small}
\end{table*}
Finally, the trade-off between area and throughput for this multi-tile deployment mode is manifested in Table~\ref{table:hw_big_vs_small}.
The maximum/mean decrease on both throughput and energy efficiency is quite significant, and do not justify the limited area gain obtain by this scheme.
Figure~\ref{fig:ppa_256_1} summarizes the per layer throughput, efficiency versus area analyses for VWW and KWS deployed in multiple $256 \times 256$ differential crossbars, graphs which can be compared against the larger deployment mode PPA characteristics reported in Figure~\ref{fig:ppa_1024_1}.


% \subsubsection{Deployment in multiple $256 \times 256$ differential crossbars}
% \label{sec:small_xbar_deployment}
\begin{figure*}[t]
    \centering
	\subfloat[Per-layer KWS efficiency dependence on throughput]{\centering
	\includegraphics[width=0.98\columnwidth]{figs/deployment_256_256/analognet-kws_small/l_eff_TOPS_l_eff_mean_TOPS_W.pdf}}
    \qquad	
    \subfloat[Per-layer VWW efficiency dependence on throughput]{\centering
    \includegraphics[width=0.98\columnwidth]{figs/deployment_256_256/analognet-vww_small/l_eff_TOPS_l_eff_mean_TOPS_W.pdf}}
%     \caption{
%     Per layer efficiency versus throughput analyses for VWW and KWS deployed in multiple $256 \times 256$ differential crossbars.
%     }
%     \label{fig:ppa_256_0}
% \end{figure}

% \begin{figure}[t]
%     \centering
	\subfloat[Per-layer KWS efficiency dependence on throughput]{\centering
	\includegraphics[width=0.98\columnwidth]{figs/deployment_256_256/analognet-kws_small/l_area_l_eff_mean_TOPS_W.pdf}}
    \qquad	
    \subfloat[Per-layer VWW efficiency dependence on throughput]{\centering
    \includegraphics[width=0.98\columnwidth]{figs/deployment_256_256/analognet-vww_small/l_area_l_eff_mean_TOPS_W.pdf}}
    \caption{
    Per layer throughput, efficiency versus area analyses for VWW and KWS deployed in multiple $256 \times 256$ differential crossbars.
    }
    \label{fig:ppa_256_1}
\end{figure*}
